Dimensionality Reduction of Longitudinal 'Omics Data using Modern Tensor Factorization

Precision medicine is a clinical approach for disease prevention, detection and treatment, which considers each individual's genetic background, environment and lifestyle. The development of this tailored avenue has been driven by the increased availability of omics methods, large cohorts of temporal samples, and their integration with clinical data. Despite the immense progression, existing computational methods for data analysis fail to provide appropriate solutions for this complex, high-dimensional and longitudinal data. In this work we have developed a new method termed TCAM, a dimensionality reduction technique for multi-way data, that overcomes major limitations when doing trajectory analysis of longitudinal omics data. Using real-world data, we show that TCAM outperforms traditional methods, as well as state-of-the-art tensor-based approaches for longitudinal microbiome data analysis. Moreover, we demonstrate the versatility of TCAM by applying it to several different omics datasets, and the applicability of it as a drop-in replacement within straightforward ML tasks.

==> child_docs/figure_panels/gfigures/postabx/S1.tex <==
\begin{supfigure}[ph!]
    \hspace*{-.25in}
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \caption{\label[sfig]{sfig:postabx.pca.baseline}}
        \includegraphics[scale=.8]{./child_docs/figure_panels/gfigures/postabx/all_baseline_pca.pdf}
    \end{subfigure}%
    \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \caption{\label[sfig]{sfig:postabx.pca.group}}
        \includegraphics[scale=.8]{./child_docs/figure_panels/gfigures/postabx/pca_all_by_group.pdf}
    \end{subfigure}%
    \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \caption{\label[sfig]{sfig:postabx.pca.group.BAS}}
        \includegraphics[scale=.8]{./child_docs/figure_panels/gfigures/postabx/postabx_pca_phase_BAS.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \caption{\label[sfig]{sfig:postabx.pca.group.ABX}}
        \includegraphics[scale=.8]{./child_docs/figure_panels/gfigures/postabx/postabx_pca_phase_ABX.pdf}
    \end{subfigure}%
    \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \caption{\label[sfig]{sfig:postabx.pca.group.INT}}
        \includegraphics[scale=.8]{./child_docs/figure_panels/gfigures/postabx/postabx_pca_phase_INT.pdf}
    \end{subfigure}\hfill%
    \begin{subfigure}[b]{0.31\textwidth}
    \hfill
    \end{subfigure}

  \caption{{\bf Comparison of \tcam with existing matrix based methods for exploratory analysis }
  \Cref{sfig:postabx.pca.baseline} PCA plot of baseline timepoints, 1-2 samples per each subjects. Points are colored according to participant.
  \Cref{sfig:postabx.pca.group} PCA plot of all timepoints. Points are colored according to group.
  \Cref{sfig:postabx.pca.group.BAS,sfig:postabx.pca.group.ABX,sfig:postabx.pca.group.INT} PCA plot of baseline, antibiotics, and intervention phases respectively. Points are colored according to group}

\end{supfigure}

\begin{supfigure}
    \begin{subfigure}[b]{1\textwidth}
        \centering
        \caption{\label[sfig]{fig:postabx.timeser.tcam}}
        \includegraphics[scale=.65]{./child_docs/figure_panels/gfigures/postabx/tcam_sp_timeser.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{1\textwidth}
      \centering
      \caption{\label[sfig]{fig:postabx.timeser.mutual}}
      \includegraphics[scale=.65]{./child_docs/figure_panels/gfigures/postabx/mutual_sp_timeser.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{1\textwidth}
        \centering
        \caption{\label[sfig]{fig:postabx.timeser.all}}
        \includegraphics[scale=.65]{./child_docs/figure_panels/gfigures/postabx/all_sp_timeser.pdf}
    \end{subfigure}
    
    \caption{{\bf Comparison of discovery rates between naive time-series analysis and \tcam based pruning}
    \Cref{fig:postabx.timeser.tcam} Time series of relative abundance levels for features discovered only when pruning the features.
    \Cref{fig:postabx.timeser.all,fig:postabx.timeser.mutual} Time series of relative abundance levels for features discovered when no pruning scheme is used (top) and by both methods (bottom).}    
\end{supfigure}
% \addtocounter{supfigure}{-1}
\pagebreak
% \begin{supcaption}[ph!]
%   \caption{{\bf Comparison of \tcam with existing matrix and tensor based methods. }
%   \Cref{sfig:postabx.pca.baseline} PCA plot of baseline timepoints, 1-2 samples per each subjects. Points are colored according to participant.
%   \Cref{sfig:postabx.pca.group} PCA plot of all timepoints. Points are colored according to group.
%   \Cref{sfig:postabx.pca.group.BAS,sfig:postabx.pca.group.ABX,sfig:postabx.pca.group.INT} PCA plot of baseline, antibiotics, and intervention phases respectively. Points are colored according to group
%   \Cref{fig:postabx.timeser.all,fig:postabx.timeser.mutual} Time series of relative abundance levels for features discovered when no pruning scheme is used (top) and by both methods (bottom).
%   \Cref{fig:postabx.timeser.tcam} Time series of relative abundance levels for features discovered only when pruning the features.
%   (~\hyperref[parpbx]{back to text})}
% \end{supcaption}
